STOP: A dataset for Spoken Task Oriented Semantic Parsing

End-to-end spoken language understanding (SLU) predicts intent directly from audio using a single model. It promises to improve the performance of assistant systems by leveraging acoustic information lost in the intermediate textual representation and preventing cascading errors from Automatic Speech Recognition (ASR). Further, having one unified model has efficiency advantages when deploying assistant systems on-device. However, the limited number of public audio datasets with semantic parse labels hinders the research progress in this area. In this paper, we release the Spoken Task-Oriented semantic Parsing (STOP) dataset, the largest and most complex SLU dataset to be publicly available. Additionally, we define low-resource splits to establish a benchmark for improving SLU when limited labeled data is available. Furthermore, in addition to the human-recorded audio, we are releasing a TTS-generated version to benchmark the performance for low-resource domain adaptation of end-to-end SLU systems. Initial experimentation show end-to-end SLU models performing slightly worse than their cascaded counterparts, which we hope encourages future work in this direction.

==> extra.tex <==
\name{%
\begin{tabular}{c}
Paden Tomasello,
Akshat Shrivastava,
Daniel Lazar,
Po-Chun Hsu,
Duc Le,
Adithya Sagar, \\
Ali Elkahky,
Jade Copet,
Wei-Ning Hsu,
Yossef Mordechay,
Robin Algayres,
Tu Ahn Nguyen, \\
Emmanuel Dupoux,
Luke Zettlemoyer,
Abdelrahman Mohamed
\end{tabular}}


\name{BLIND}
\address{BLIND}
%\address{Author Affiliation(s)}
%\address{Meta AI}

\subsection{ Demographic Analysis }

We evaluate our best model (HuBERT using both audio and ASR pretraining) on a variety of subsplits in order to understand the shortcomings of end-to-end NLU. 

Table \ref{tab:gender_error} shows our results on Male and Female only speakers. We do not show results on Non-binary as there are not enough samples to make it statistically significant. As can be seen, our end-to-end system performs equally well on Male and Female identified speakers. Table \ref{tab:native_english_stats} shows our results split on native and non-native English speakers. Surprisingly, our model actually performs slightly better on Nonnative English speakers for the EM metric than on native english speakers. These results give us a good indication that our dataset is robust to both gender and non-native english speakers. 



\subsection{Domain Analysis}

Table \ref{tab:domain_error} shows how our best model performs across different domains. As can be seen, the worst domains for EM accuracy are messaging and reminder, but the model actually performs decently on these domains in Tree accuracy. These results tell us that for messaging and reminder, the model is generally able to understand the intent of the command, but struggles to transcribe the audio perfectly. This makes sense intuitively, since navigation and reminder has a wide range of possibilities for the intent slots and are more challenging to transcribe. 

For Tree Accuracy, the worse performing domains are music, navigation, and timer. We see some correlation with poor accuracy and the number of intents for a domain: music navigation and timer have 15, 17, 11 possible types of intents, where the highest performing domain, weather and messaging has only 7 intents. 


\begin{table}[t]
  \caption{ Domain Error Analysis}
  \label{tab:domain_error}
  \centering
  \begin{tabular}{lcc}
    \toprule
    Model & EM & Tree\\
    \midrule
    E2E & alarm & 79.20 & 86.73 \\
    Cascaded (STOP) & alarm & 81.48 & 87.16 \\
    Cascaded (Librispeech) & alarm & 36.62 & 65.56 \\
    Text GT & alarm & 85.62 & 88.00 \\
    E2E & event & 65.17 & 81.51 \\
    Cascaded (STOP) & event & 63.98 & 84.99 \\
    Cascaded (Librispeech) & event & 17.88 & 60.49 \\
    Text GT & event & 80.26 & 88.64 \\
    E2E & messaging & 49.52 & 89.21 \\
    Cascaded (STOP) & messaging & 55.75 & 91.67 \\
    Cascaded (Librispeech) & messaging & 24.95 & 70.66 \\
    Text GT & messaging & 93.19 & 95.32 \\
    E2E & music & 69.56 & 77.32 \\
    Cascaded (STOP) & music & 70.97 & 80.18 \\
    Cascaded (Librispeech) & music & 38.01 & 56.67 \\
    Text GT & music & 80.39 & 81.79 \\
    E2E & navigation & 64.18 & 77.86 \\
    Cascaded (STOP) & navigation & 67.47 & 81.27 \\
    Cascaded (Librispeech) & navigation & 31.89 & 59.95 \\
    Text GT & navigation & 82.39 & 83.53 \\
    E2E & reminder & 56.84 & 81.29 \\
    Cascaded (STOP) & reminder & 62.44 & 86.79 \\
    Cascaded (Librispeech) & reminder & 20.90 & 61.78 \\
    Text GT & reminder & 85.23 & 89.07 \\
    E2E & timer & 73.47 & 77.68 \\
    Cascaded (STOP) & timer & 81.83 & 84.76 \\
    Cascaded (Librispeech) & timer & 48.80 & 58.57 \\
    Text GT & timer & 84.01 & 85.51 \\
    E2E & weather & 83.83 & 90.37 \\
    Cascaded (STOP) & weather & 83.39 & 91.70 \\
    Cascaded (Librispeech) & weather & 27.44 & 53.35 \\
    Text GT & weather & 90.81 & 93.14 \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[h]
  \caption{ Gender Error Analysis}
  \label{tab:gender_error}
  \centering
  \begin{tabular}{lcc|cc}
    \toprule
    & \multicolumn{2}{c}{Male} & \multicolumn{2}{c}{Female} \\
    \midrule
    & EM & Tree & EM & Tree \\
    \midrule
    End-to-end NLU & 69.75 & 82.81 & 69.12 & 82.83 \\
    \midrule
    Cascaded System (STOP) & 73.08 & 85.75 & 71.28 & 85.70 \\
    Cascaded System (Librispeech) & 31.76 & 60.87 & 30.67 & 60.38 \\
    Text GT & 85.05 & 87.78 & 85.54 & 87.95 \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[t]
  \caption{ Native English Error Analysis}
  \label{tab:native_error}
  \centering
  \begin{tabular}{lcc|cc}
    \toprule
    & \multicolumn{2}{c}{Native English} & \multicolumn{2}{c}{Nonnative English} \\
    \midrule
    & EM & Tree & EM & Tree \\
    \midrule
    End-to-end NLU & 69.02 & 82.76 & 70.78 & 82.92 \\
    \midrule
    Cascaded System (STOP) & 72.37 & 85.78 & 72.33 & 84.82 \\
    Cascaded System (Librispeech) & 31.64 & 61.41 & 26.56 & 49.94 \\
    Text GT & 85.19 & 87.80 & 85.58 & 87.92 \\
    \bottomrule
  \end{tabular}
\end{table}


\begin{table*}[hb]
    \centering
    \begin{tabular}{l|cccccccccc}
        \toprule
         \textbf{Experiment} & TTS Only & 10spis & 25spis & 50spis & 100 spis & 250spis & 500spis & 1000spis \\
        \midrule
         Low-resource Baseline \\
         TTS Augmented - Low-resource \\
         Domain Adaptation \\
         TTS Augmented - Domain Adaptation
    \end{tabular}
    \caption{A comparison of low-resource and domain adaptation ablation studies for the reminder domain }
    \label{tab:tts-low-resource-domain-adaptation-experiment-reminder}
\end{table*}

\begin{table*}[hb]
    \centering
    \begin{tabular}{l|cccccccccc}
        \toprule
         \textbf{Experiment} & TTS Only & 10spis & 25spis & 50spis & 100 spis & 250spis & 500spis & 1000spis \\
        \midrule
         Low-resource Baseline\\
         TTS Augmented - Low-resource \\
         Domain Adaptation\\
         TTS Augemented - Domain Adaptation
    \end{tabular}
    \caption{A comparison of low-resource and domain adaptation ablation studies for the weather domain }
    \label{tab:tts-low-resource-domain-adaptation-experiment-weather}
\end{table*}


\begin{table*}[ht]
    \centering
    \begin{tabular}{p{0.5\linewidth}|p{0.5\linewidth}}
        \textbf{Utterance} & \textbf{Spoken Text Normalization} \\
        \toprule
         can you play 80s alternative only  & can you play eighties alternative only \\
        \midrule
        Wake me at 7am &  Wake me at seven am \\
        \midrule
        Find the time to Key West using I-10, \& I-57. & Find the time to key west using I ten and I fifty seven \\
        \midrule
        Is it going to be below 95 in degrees F in San Francisco & Is it going to be below ninety five in degrees fahrenheit in San Francisco \\
        \midrule
    \end{tabular}
    \caption{Example normalizations. On the left, are the original TOPv2 Utterances. On the right is the text normalization choosen by our normalization system}
    \label{tab:text_normalization}
\end{table*}


\begin{table}[ht]
    \centering
    \begin{tabular}{p{0.9\linewidth}}
        \toprule
        initial utterances \\
        \textbf{98121 on 3rd ave after I-90 exit // I spent 405 dollars} \\
        \toprule
        \toprule
        ninety eight thousand one hundred and twenty one on third ave after I-nine oh exit // I spent four oh five dollars \\
        \midrule
        ninety eight thousand on hundred twenty one on third ave after I-ninety exist // I spent four oh five dollars \\
        \midrule
        ninety eight thousand one hundred twenty one on third ave after I-nine oh exist // I spent four hundred five dollars \\
        \midrule
        ninety eight thousand one hundred twenty one on third ave after I-nintey  // I spent four hundred five dollars \\
        \midrule
        nine eight one two one on third ave after I-nine // I spent four oh five dollars \\
        \midrule
        nine eight one two one on third ave after I-ninety exist // I spent four oh five dollars
        
    \end{tabular}
    \caption{ Two examples showing the differenct normalizations that might be produced for a given utterance }
    \label{tab:normalization_enumeration}
\end{table}


\begin{table}[h]
  \caption{ Gender Statistics  }
  \label{tab:gender_stats}
  \centering
  \begin{tabular}{l | cccc}
    \toprule
    \textbf{Split} & \textbf{Female} & \textbf{Male} & \textbf{Non-binary} & \textbf{Unanswered} \\
    \midrule
    Full & 44.55\% & 54.62\% &  0.79\%  & 0.04\% \\
    Train & 55.54\% & 43.03\% & 1.42\% & 0.02\% \\
    Eval & 58.52\% & 40.97\% & 0.30 \% & 0.20 \% \\
    Test &  40.82\%  & 59.18\% &  0.00 \% & 0.00\% \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[h]
  \caption{ Native English Statistics }
  \label{tab:native_english_stats}
  \centering
  \begin{tabular}{l | ccc}
    \toprule
    \textbf{Split} & \textbf{Native} & \textbf{Nonnative} & \textbf{Prefer not to say}  \\
    \midrule
    Full & 95.18\% & 4.09\% & 0.73\% \\
    \midrule
    Train & 97.78\% & 1.83\% & 0.39\% \\
    \midrule
    Eval & 93.86\% & 6.14\% & 0.00\%  \\
    \midrule
    Test & 91.62\% & 6.80\% & 1.59\% \\
    \bottomrule
  \end{tabular}
\end{table}
